Sparse Uncertainty Representation in Deep Learning with Inducing Weights

Bayesian neural networks and deep ensembles represent two modern paradigms of uncertainty quantification in deep learning. Yet these approaches struggle to scale mainly due to memory inefficiency issues, since they require parameter storage several times higher than their deterministic counterparts. To address this, we augment the weight matrix of each layer with a small number of inducing weights, thereby projecting the uncertainty quantification into such low dimensional spaces. We further extend Matheron's conditional Gaussian sampling rule to enable fast weight sampling, which enables our inference method to maintain reasonable run-time as compared with ensembles. Importantly, our approach achieves competitive performance to the state-of-the-art in prediction and uncertainty estimation tasks with fully connected neural networks and ResNets, while reducing the parameter size to $\leq 24.3\%$ of that of a $single$ neural network.

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please read the checklist guidelines carefully for information on how to answer these questions.
% For each question, change the default \answerTODO{} to \answerYes{}, \answerNo{}, or \answerNA{}.
% You are strongly encouraged to include a {\bf justification to your answer}, either by referencing the appropriate section of your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your answers.
% Note that the Checklist section does not count towards the page limit.
% In your paper, please delete this instructions block and only keep the Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{(Our work considers reducing model parameter sizes for Bayesian neural networks.)}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{(this is for the corrupted CIFAR dataset \citep{hendrycks2019benchmarking}.)}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> inducing_weight_old.tex <==
\subsection{Inducing weights for neural network parameters}
\label{sec:inducing}

Following the design principles of inducing variables, we introduce a set of \emph{inducing weights} to assist uncertainty estimation in neural networks. In detail, we augment each network layer $l$ with a \emph{smaller} inducing weight matrix $\inducing_l$, and construct joint prior/approximate posterior distributions for inference. In the rest of the paper we assume a factorised prior across layers $p(\allweights) = \prod_{l}p(\weight_l)$, and for notation ease we drop the $l$ indices when the context is clear. 

\vspace{-0.5em}
\paragraph{Augmenting network layers with inducing weights}
Suppose the weight $\weight \in \mathbb{R}^{d_{in} \times d_{out}}$ has a Gaussian prior $p(\weight) = p(\vect(\weight)) = \gauss(0, \sigma^2 \eye)$ where $\vect(\weight)$ concatenates the columns of the weight matrix into a vector.
Our first attempt is to augment $p(\vect(\weight))$ with an inducing weight variable $\inducing \in \mathbb{R}^{M_{out} \times M_{in}}$, resulting in a joint Gaussian prior:
\begin{align}
    \pmat{\vect(\weight)\\\vect(\inducing)} \sim p(\vect(\weight), \vect(\inducing)) := \gauss(\bm{0}, \fullcov)
    \quad \text{such that }
    \fullcov = \pmat{\sigma^2\eye & \Sigma_{\weight \inducing} \\ \Sigma_{\inducing \weight} & \Sigma_{\inducing \inducing}}.
\end{align}
%
It is clear that the marginalisation constraint (\ref{eq:marginalisation_constraint}) is satisfied for any configurations of $\Sigma_{\weight \inducing}$, $\Sigma_{\inducing \weight}$ and $\Sigma_{\inducing \inducing}$, as long as both $\Sigma$ and $\Sigma_{\inducing \inducing}$ are positive definite.

\vspace{-0.5em}
\paragraph{Posterior approximation in the joint space}
We construct a factorised posterior approximation across the layers: $q(\allweights, \allinducing) = \prod_l q(\weight_l, \inducing_l)$. Within each layer, we define $q(\weight, \inducing) = q(\weight | \inducing) q(\inducing)$.
%
The simplest option for $q(\weight\given\inducing)$ is $q(\weight\given\inducing) = p(\vect(\weight)\given\vect(\inducing)) = \gauss(\mu_{\weight\given\inducing}, \Sigma_{\weight\given\inducing})$, similar to sparse GPs.
A slightly more flexible variant rescales the covariance matrix while keeping the mean tied, i.e. $q(\weight\given\inducing) = q(\vect(\weight)\given\vect(\inducing)) = \gauss(\mu_{\weight\given\inducing}, \lambda^2 \Sigma_{\weight\given\inducing})$, which still allows for the KL term to be calculated efficiently (see Appendix \ref{app:kl_divergence_derivation}):
\begin{align}
    R(\lambda) := \kl\left[ q(\weight\given\inducing) \vert\vert p(\weight\given\inducing ) \right] = d_{in} d_{out} (0.5\lambda^2 - \log \lambda - 0.5), \quad \weight \in \mathbb{R}^{d_{out} \times d_{in}}.
\label{eq:conditional_kl}
\end{align}
Plugging $\theta = \{ \allweights \}, a = \{ \allinducing \}$ in to (\ref{eq:inducing_elbo_general}) results in the following variational lower-bound
\begin{align}
    \mathcal{L}(q(\allweights, \inducing_{1:L})) &= \mathbb{E}_{q(\allweights)}[\log p(\data | \allweights)] - \textstyle\sum\nolimits_{l=1}^L (R(\lambda_l) + \kl[q(\inducing_l) || p(\inducing_l)]), \label{eq:elbo_inducing_weight_reduced}
\end{align}
with $\lambda_l$ the associated scaling parameter for $q(\weight_l | \inducing_l)$. We also see that $\Sigma_{\weight \inducing}$, $\Sigma_{\inducing \weight}$ and $\Sigma_{\inducing \inducing}$ are in fact variational parameters which are optimised using the variational lower-bound. 

\paragraph{Two choices of $q(\inducing)$}
A simple choice is FFG $q(\vect(\inducing)) = \gauss(\bm{m}_u, \text{diag}(\bm{v}_u))$, which performs mean-field inference in $\inducing$ space \citep[c.f.][]{blundell2015weight}, and in this case $\kl[q(\inducing) || p(\inducing)]$ has a closed-form solution.
%
Another choice is a ``mixture of delta measures'' $q(\inducing) = \frac{1}{K}\sum_{k=1}^K \delta(\inducing = \inducing^{(k)})$. This approach can be viewed as constructing ``deep ensembles'' in $\inducing$ space, and we follow ensemble methods \citep[e.g.][]{lakshminarayanan2017simple} to drop $\kl[q(\inducing) || p(\inducing)]$ in (\ref{eq:elbo_inducing_weight_reduced}). %

Often the inducing weight $\inducing$ is chosen to have significantly lower dimensions compared to $\weight$. Combining with the fact that $q(\weight|\inducing)$ and $p(\weight | \inducing)$ only differ in the covariance scaling constant, we see that $\inducing$ can be regarded as a \emph{sparse representation of uncertainty} for the network layer, as the major updates in (approximate) posterior belief is quantified by $q(\inducing)$.
Next we will introduce the details of $p(\weight, \inducing)$, as well as the efficient computation achieved by our design.


\subsection{Efficient parameterization with matrix normals}
\label{sec:matrix_normal_inducing}

Similar to sparse GPs, the inducing weights should enable efficient parameterisation of $q(\weight, \inducing)$. However, as $\text{dim}(\vect(\weight))$ is typically large (e.g. of the order of $10^5-10^7$), using a full covariance Gaussian for $q(\vect(\weight), \vect(\inducing))$ becomes computationally intractable. 
%
Fortunately, this issue can be addressed using matrix normal distributions. Notice that the prior $p(\vect(\weight)) = \gauss(\bm{0}, \sigma^2 I)$ has an equivalent matrix normal distribution form as $p(\weight) = \matgauss(0, \sigma_r^2 \eye, \sigma_c^2 \eye)$, with $\sigma_r, \sigma_c > 0$ the row and column standard deviations satisfying $\sigma = \sigma_r\sigma_c$.
%
Now we introduce the inducing variables in matrix space, in addition to $\inducing$ we pad in two auxiliary variables $\inducing_r \in \mathbb{R}^{M_{out} \times d_{in}}$, $\inducing_c \in \mathbb{R}^{d_{out} \times M_{in}}$ (see Figure \ref{fig:visualisation_matheron}(a) for a visualisation), so that the full augmented prior is:
%\CZ{considering color some of the variable notation. For example color $\Sigma_r$ all in green etc in all equations. It helps to read the equations, especially when there are many equations involving same variables. May be also consider the choice of color, for example, everthing relating to r in warm color (red, orange, peach, brown) and relating to c in cold colr (blue, green etc)}
%
\begin{align}
    \pmat{\weight & \inducing_c\\\inducing_r & \inducing} \sim p(\weight, \inducing_c, \inducing_r, \inducing) &:= \matgauss(0, \fullcov_r, \fullcov_c), \label{eq:inducing_full_joint}\\
    \text{with}\quad
    \inducingchol_r = \pmat{\sigma_r \eye & 0\\\covparam_r & \precparam_r}
    \quad\text{s.t.}\quad
    \fullcov_r &= \inducingchol_r\inducingchol_r^\top = \pmat{\sigma_r^2\eye & \sigma_r \covparam_r^\top\\\sigma_r \covparam_r & \covparam_r\covparam_r^\top + \precparam_r^2},\nonumber\\
    \text{and}\quad
    \inducingchol_c = \pmat{\sigma_c \eye & 0\\\covparam_c & \precparam_c}
    \quad\text{s.t.}\quad
    \fullcov_c &= \inducingchol_c\inducingchol_c^\top = \pmat{\sigma_c^2\eye & \sigma_c\covparam_c^\top\\\sigma_c\covparam_c & \covparam_c\covparam_c^\top + \precparam_c^2}.\nonumber
\end{align}
%
Matrix normal distributions have similar marginalization and conditioning properties as multivariate Gaussian distributions. Therefore the marginalisation constraint (\ref{eq:marginalisation_constraint}) is satisfied for any $\covparam_c, \covparam_r$, $\precparam_c$ and $\precparam_r$, so that they can be optimised, meaning that the variational parameters are now $\phi = \{\covparam_c, \covparam_r, \precparam_c, \precparam_r, \lambda, \text{dist.~params.~of } q(\inducing) \}$ for each network layer.  
%
The marginal distribution of the inducing weight is $p(\inducing) = \matgauss(0, \inducingcov_r, \inducingcov_c)$ with $\inducingcov_r = \covparam_r\covparam_r^\top + \precparam_r^2$ and $\inducingcov_c = \covparam_c\covparam_c^\top + \precparam_c^2$. In experiments we use \emph{whitened} inducing weights which transforms $\inducing$ so that $p(\inducing) = \matgauss(0, I, I)$ (Appendix \ref{app:hierarchical_inducing}), but for clarity, in the main text we remain using the formulas presented above.

The matrix normal parameterisation introduces two additional variables $\inducing_r, \inducing_c$ without providing additional expressiveness.
Hence it is desirable to integrate them out, leading to a joint multivariate normal with Khatri-Rao product structure (i.e.~blocks of Kronecker products) for the covariance:
%
\begin{equation}
    p(\vect(\weight), \vect(\inducing)) = \gauss \left(0, \pmat{\sigma_c^2 \eye \kron \sigma_r^2 \eye & \sigma_c\covparam_c^\top \kron \sigma_r\covparam_r^\top\\\sigma_c\covparam_c \kron \sigma_r\covparam_r & \inducingcov_c \kron \inducingcov_r} \right),
\end{equation}
%
In other words $\Sigma_{\inducing \weight} = \sigma_c\covparam_c \kron \sigma_r\covparam_r$ and $\Sigma_{\inducing \inducing} = \inducingcov_c \kron \inducingcov_r$.
%
So while the marginals $p(\weight)$, $p(\inducing)$ and the full joint $p(\weight, \inducing_c, \inducing_r, \inducing)$ have efficient matrix normal forms, the joint $p(\weight, \inducing)$ and the conditionals $p(\weight | \inducing)$, $q(\weight | \inducing)$ do not. Hence \emph{direct} sampling from $q(\weight | \inducing)$ remains prohibitively expensive as it requires computing the Cholesky decompostion of the conditional covariance $\lambda^2 \Sigma_{\weight\given\inducing}$. In the next section we introduce an efficient sampling trick for $q(\weight | \inducing)$ which avoids computing Cholesky decomposition of $\lambda^2 \Sigma_{\weight\given\inducing}$ in the price of small additional noise variances.

==> tables/full_uncertainty_backup.tex <==
\toprule
& \multicolumn{4}{c}{CIFAR10}& \multicolumn{4}{c}{CIFAR100}\\
Method & Acc. $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & Brier $\downarrow$ & Acc. $\uparrow$ & NLL $\downarrow$ & ECE $\downarrow$ & Brier $\downarrow$\\
\midrule
Deterministic & $94.72{\scriptstyle {\pm} 0.08}$ & $0.43{\scriptstyle {\pm} 0.01}$ & $4.46{\scriptstyle {\pm} 0.08}$ & $0.10{\scriptstyle {\pm} 0.00}$ & $75.73{\scriptstyle {\pm} 0.16}$ & $2.14{\scriptstyle {\pm} 0.01}$ & $19.69{\scriptstyle {\pm} 0.15}$ & $0.43{\scriptstyle {\pm} 0.00}$\\
Ensemble-W & $95.90{\scriptstyle \phantom{{\pm} 0.00}}$ & $0.20{\scriptstyle \phantom{{\pm} 0.00}}$ & $1.08{\scriptstyle \phantom{{\pm} 0.00}}$ & $0.06{\scriptstyle \phantom{{\pm} 0.00}}$ & $79.33{\scriptstyle \phantom{{\pm} 0.00}}$ & $1.23{\scriptstyle \phantom{{\pm} 0.00}}$ & $6.51{\scriptstyle \phantom{{\pm} 0.00}}$ & $0.31{\scriptstyle \phantom{{\pm} 0.00}}$\\
FFG-W & $94.13{\scriptstyle {\pm} 0.08}$ & $0.18{\scriptstyle {\pm} 0.00}$ & $0.50{\scriptstyle {\pm} 0.06}$ & $0.09{\scriptstyle {\pm} 0.00}$ & $74.44{\scriptstyle {\pm} 0.27}$ & $1.01{\scriptstyle {\pm} 0.01}$ & $4.24{\scriptstyle {\pm} 0.10}$ & $0.35{\scriptstyle {\pm} 0.00}$\\
FFG-U (M=64) & $94.40{\scriptstyle {\pm} 0.05}$ & $0.17{\scriptstyle {\pm} 0.00}$ & $0.64{\scriptstyle {\pm} 0.06}$ & $0.08{\scriptstyle {\pm} 0.00}$ & $75.37{\scriptstyle {\pm} 0.09}$ & $0.92{\scriptstyle {\pm} 0.01}$ & $2.29{\scriptstyle {\pm} 0.39}$ & $0.34{\scriptstyle {\pm} 0.00}$\\
FFG-U (M=128) & $94.66{\scriptstyle {\pm} 0.09}$ & $0.17{\scriptstyle {\pm} 0.00}$ & $1.59{\scriptstyle {\pm} 0.06}$ & $0.08{\scriptstyle {\pm} 0.00}$ & $75.88{\scriptstyle {\pm} 0.13}$ & $0.91{\scriptstyle {\pm} 0.00}$ & $6.66{\scriptstyle {\pm} 0.15}$ & $0.34{\scriptstyle {\pm} 0.00}$\\
Ensemble-U (M=64) & $94.94{\scriptstyle {\pm} 0.07}$ & $0.16{\scriptstyle {\pm} 0.00}$ & $0.45{\scriptstyle {\pm} 0.06}$ & $0.08{\scriptstyle {\pm} 0.00}$ & $75.97{\scriptstyle {\pm} 0.12}$ & $0.90{\scriptstyle {\pm} 0.00}$ & $1.12{\scriptstyle {\pm} 0.06}$ & $0.33{\scriptstyle {\pm} 0.00}$\\
Ensemble-U (M=128) & $95.34{\scriptstyle {\pm} 0.05}$ & $0.17{\scriptstyle {\pm} 0.00}$ & $1.29{\scriptstyle {\pm} 0.05}$ & $0.07{\scriptstyle {\pm} 0.00}$ & $77.61{\scriptstyle {\pm} 0.11}$ & $0.94{\scriptstyle {\pm} 0.00}$ & $6.00{\scriptstyle {\pm} 0.12}$ & $0.32{\scriptstyle {\pm} 0.00}$\\
\bottomrule

